Evaluating the Security of Aircraft Systems

The sophistication and complexity of cyber attacks and the variety of targeted platforms have been growing in recent years. Various adversaries are abusing an increasing range of platforms, e.g., enterprise platforms, mobile phones, PCs, transportation systems, and industrial control systems. In recent years, we have witnessed various cyber attacks on transportation systems, including attacks on ports, airports, and trains. It is only a matter of time before transportation systems become a more common target of cyber attackers. Due to the enormous potential damage inherent in attacking vehicles carrying many passengers and the lack of security measures applied in traditional airborne systems, the vulnerability of aircraft systems is one of the most concerning topics in the vehicle security domain. This paper provides a comprehensive review of aircraft systems and components and their various networks, emphasizing the cyber threats they are exposed to and the impact of a cyber attack on these components and networks and the essential capabilities of the aircraft. In addition, we present a comprehensive and in-depth taxonomy that standardizes the knowledge and understanding of cyber security in the avionics field from an adversary's perspective. The taxonomy divides techniques into relevant categories (tactics) reflecting the various phases of the adversarial attack lifecycle and maps existing attacks according to the MITRE ATT&CK methodology. Furthermore, we analyze the security risks among the various systems according to the potential threat actors and categorize the threats based on STRIDE threat model. Future work directions are presented as guidelines for industry and academia.

==> Tables/table_draft.tex <==
\begin{table}[ht!]
\centering
\tiny
\begin{tabular}{
|m{0.1\textwidth}
|m{0.1\textwidth}5
|m{0.1\textwidth}
|m{0.1\textwidth}
|m{0.1\textwidth}
|m{0.1\textwidth}
|m{0.1\textwidth}
|m{0.1\textwidth}
|m{0.1\textwidth}
|m{0.1\textwidth}
|m{0.1\textwidth}
|m{0.1\textwidth}
|m{0.1\textwidth}
|m{0.1\textwidth}
|m{0.1\textwidth}
|m{0.1\textwidth}
|m{0.1\textwidth}
|m{0.1\textwidth}
|m{0.1\textwidth}
|m{0.1\textwidth}
|m{0.1\textwidth}
|m{0.1\textwidth}
|m{0.1\textwidth}
|m{0.1\textwidth}
|m{0.1\textwidth}
|m{0.1\textwidth}
|m{0.1\textwidth}
|m{0.1\textwidth}
|m{0.1\textwidth}
|m{0.1\textwidth}
|m{0.1\textwidth}
|m{0.1\textwidth}
|m{0.1\textwidth}
|m{0.1\textwidth}
|m{0.1\textwidth}|}
\Xhline{2pt}

\textbf{Paper} &
\multicolumn{32}{c}{\textbf{Target Assets}} &
\textbf{Security threats} &
\textbf{Taxonomy} \\ 

    &
    \multicolumn{3}{c}\textbf{Communication systems} &
    \multicolumn{8}{c}\textbf{Navigation systems} &
    \multicolumn{4}{c}\textbf{Surveillance systems} &
    \multicolumn{5}{c}\textbf{Information and alerting systems} &
    \multicolumn{8}{c}\textbf{Backend avionics and network components} &
    \multicolumn{4}{c}\textbf{Systems' connectivity's}  & & & \\
    
    &
    & \rotatebox{90}{SATCOM}
    & \rotatebox{90}{CPDLC}
    & \rotatebox{90}{ACARS}
    
    & \rotatebox{90}{DME}
    & \rotatebox{90}{VOR}
    & \rotatebox{90}{NDB}
    & \rotatebox{90}{ILS}
    & \rotatebox{90}{DNNSS}
    & \rotatebox{90}{ABAS}
    & \rotatebox{90}{SBAS}
    & \rotatebox{90}{GNAS}
    
    & \rotatebox{90}{PSR}
    & \rotatebox{90}{SSR}
    & \rotatebox{90}{MLAT}
    & \rotatebox{90}{ADS-B}
    
    & \rotatebox{90}{TCAS}
    & \rotatebox{90}{ACAS X}
    & \rotatebox{90}{Engine Alerting}
    & \rotatebox{90}{FIS-B}
    & \rotatebox{90}{TIS-B}
    
    & \rotatebox{90}{EFB}
    & \rotatebox{90}{TWLU}
    & \rotatebox{90}{CWLU}
    & \rotatebox{90}{EGM}
    & \rotatebox{90}{NIM}
    & \rotatebox{90}{CSS}
    & \rotatebox{90}{FDR}
    & \rotatebox{90}{CIS-MS}
    
    & \rotatebox{90}{ACD}
    & \rotatebox{90}{AISD}
    & \rotatebox{90}{PIESD}
    & \rotatebox{90}{External Networks} & &\\
\Xhline{2pt}
\cite{elmarady2021studying}                                  & CPDLC, ACARS                              & DME, VOR, GNSS, ILS                              & PSR, SSR, MLAT, ADS-B                    & \xmark                                & \xmark                            & \xmark                        & Likelihood and impact analysis                                                              & \xmark                             \\ 
\hline
\cite{dave2022cyber}                                    & SATCOM, CPDLC, ACARS                      & DME, VOR, GNSS, ILS                              & PSR, SSR, ADS-B                          & \xmark                                & \xmark                            & \xmark                        & outline attack's goal using CIA triad                                                                                    & \xmark                             \\ 
\hline
\cite{strohmeier2016perception}                                      & CPDLC. ACARS                              & DME, VOR, NDB, ILS                               & PSR, SSR, MLAT, ADS-B                    & TCAS, FIS-B, TIS-B                                   & \xmark                            & \xmark                        & Security impact according to pilot\par{}~and controller response to severalattacks (survey) & \xmark                             \\ 
\hline
{\cellcolor[rgb]{0.988,0.988,0.988}}\cite{lykou2019aviation} & SATCOM                                    & GNSS                                             & PSR, SSR, ADS-B                          & TCAS, FIS-B, TIS-B                                   & \xmark                            & \xmark                        & Categorized actors in relation to their resources and motivations                           & \xmark                             \\ 
\hline
\cite{shaikh2019review}                                      & CPDLC, ACARS                              & GNSS                                             & ADS-B                                    & \xmark                                & \xmark                            & \xmark                        & \xmark                                                                       & \xmark                             \\ 
\hline
\cite{strohmeier2020securing}                                      & CPDLC, ACARS                              & \xmark                            & SSR, ADS-B, MLAT                         & TCAS                                & \xmark                            & \xmark                        & Examining realistic events and accidents that have occurred                                                                      & \xmark                             \\

\Xhline{2pt}
The proposed security analysis& SATCOM, CPDLC, ACARS                      & DME, VOR, NDB, ILS, GNSS, ABAS, SBAS, GNAS & PSR, SSR, MLAT, ADS-B                    & TCAS, ACAS X, Engine Alerting, FIS-B, TIS-B          & EFB, TWLU, CWLU, EGM, NIM, CSS, FDR,CIS-MS & ACD, AISD, PIESD, and external networks & Actors capabilities, \par{}STRIDE model                                                     & ATT\&CK extension and case studies  \\ 
\Xhline{2pt}


\end{tabular}

\caption{Comparison of the proposed threat analysis with existing aviation security surveys}
\label{tab:capa}
\end{table}
